Molecular Hypergraph Grammar with its Application to Molecular Optimization

Molecular optimization aims to discover novel molecules with desirable properties. Two fundamental challenges are: (i) it is not trivial to generate valid molecules in a controllable way due to hard chemical constraints such as the valency conditions, and (ii) it is often costly to evaluate a property of a novel molecule, and therefore, the number of property evaluations is limited. These challenges are to some extent alleviated by a combination of a variational autoencoder (VAE) and Bayesian optimization (BO). VAE converts a molecule into/from its latent continuous vector, and BO optimizes a latent continuous vector (and its corresponding molecule) within a limited number of property evaluations. While the most recent work, for the first time, achieved 100% validity, its architecture is rather complex due to auxiliary neural networks other than VAE, making it difficult to train. This paper presents a molecular hypergraph grammar variational autoencoder (MHG-VAE), which uses a single VAE to achieve 100% validity. Our idea is to develop a graph grammar encoding the hard chemical constraints, called molecular hypergraph grammar (MHG), which guides VAE to always generate valid molecules. We also present an algorithm to construct MHG from a set of molecules.

==> figs/bo_mols/test.tex <==
\begin{figure}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/0.pdf}
5.558
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/1.pdf}
5.401
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/2.pdf}
5.344
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/3.pdf}
5.289
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/4.pdf}
5.063
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/5.pdf}
4.979
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/6.pdf}
4.811
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/7.pdf}
4.779
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/8.pdf}
4.775
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/9.pdf}
4.730
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/10.pdf}
4.712
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/11.pdf}
4.641
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/12.pdf}
4.617
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/13.pdf}
4.598
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/14.pdf}
4.595
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/15.pdf}
4.555
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/16.pdf}
4.546
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/17.pdf}
4.538
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/18.pdf}
4.484
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/19.pdf}
4.464
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/20.pdf}
4.450
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/21.pdf}
4.443
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/22.pdf}
4.408
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/23.pdf}
4.404
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/24.pdf}
4.374
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/25.pdf}
4.362
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/26.pdf}
4.354
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/27.pdf}
4.351
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/28.pdf}
4.349
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/29.pdf}
4.341
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/30.pdf}
4.335
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/31.pdf}
4.294
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/32.pdf}
4.274
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/33.pdf}
4.265
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/34.pdf}
4.259
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/35.pdf}
4.258
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/36.pdf}
4.242
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/37.pdf}
4.240
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/38.pdf}
4.233
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/39.pdf}
4.209
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/40.pdf}
4.202
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/41.pdf}
4.196
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/42.pdf}
4.185
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/43.pdf}
4.171
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/44.pdf}
4.169
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/45.pdf}
4.163
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/46.pdf}
4.153
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/47.pdf}
4.150
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/48.pdf}
4.124
\end{minipage}
\begin{minipage}{.24\hsize}
\centering
\includegraphics[width=\hsize]{figs/bo_mols/49.pdf}
4.124
\end{minipage}
\end{figure}

